Skeins, clusters and wavefunctions

In previous work of the second- and third-named authors with Linhui Shen, cluster theory was used to construct wavefunctions for branes in threespace and conjecturally relate them to open Gromov-Witten invariants. This was done by defining a quantum Lagrangian subvariety of a quantum cluster variety, and mutating a simple solution to the defining equations in a distinguished seed. In this paper, we extend the construction to incorporate the skein-theoretic approach to open Gromov-Witten theory of Ekholm-Shende. In particular, we define a skein-theoretic version of cluster theory, including the groupoid of seeds and mutations and a skein-theoretic version of the quantum dilogarithm. We prove a pentagon relation in the skein of the closed torus in this context, and give strong evidence that its analogue holds for arbitrary surfaces. We propose face relations satisfied by the skein-theoretic wavefunction, prove their invariance under mutations, and show their solution is unique. We define a skein version of framings in the story, and use the novel cluster structure to compute wavefunctions in several examples. The skein approach incorporates moduli spaces of sheaves of higher microlocal rank and their quantizations.

==> Globalization.tex <==
\iffalse
\subsection{Globalization}
\label{sec:globalization}
\red{We now show that $\Gamma$ labels a cluster chart $\cP_\Gamma$ of a global moduli space $\cP$ with a global Lagrangian $\cM$ such that in each chart $\cM\cap \cP_\Gamma = \cM_\Gamma.$} 
We begin by considering a more general space.

\fi


%\subsection{Example: the moduli space $\cX_{PGL_2, S_{g+3}}$}

 %Let $\mathcal{T}$ be an ideal triangulation of $S_{g+3}$, i.e., a triangulation with vertices at the punctures. 






\begin{example} \label{rmk:special.case} 
Let $G=PGL_2$.
The following triangulations show an example of involution for a sphere with 4 punctures.


\begin{center}
\begin{tikzpicture}[scale=0.9]
\node at (0,0) {$\bullet$};
\node at (2,0) {$\bullet$};
\node at (0,2) {$\bullet$};
\node at (2,2) {$\bullet$};
\draw (0,0)--(2,0)--(2,2)--(0,2)--cycle;
\draw [dashed] (0,0) --(2,2);
\draw (2,0)--(0,2);
\node at (-0.2, 1) {$w$};
\node at (1, 2.2) {$x$};
\node at (2.2, 1) {$y$};
\node at (1, -0.2) {$z$};
\node at (1.5, 1.3) {$u$};
\node at (0.5, 1.3) {$v$};
\node at(4.25, 1.2) {${\rm reflection}$};
\draw[thick, -latex] (3,1)--(5.5,1);
\end{tikzpicture}
\begin{tikzpicture}[scale=0.9]
\node at (0,0) {$\bullet$};
\node at (2,0) {$\bullet$};
\node at (0,2) {$\bullet$};
\node at (2,2) {$\bullet$};
\draw (0,0)--(2,0)--(2,2)--(0,2)--cycle;
\draw (0,0) --(2,2);
\draw[dashed] (2,0)--(0,2);
\node at (-0.2, 1) {$w^{-1}$};
\node at (1, 2.2) {$x^{-1}$};
\node at (2.2, 1) {$y^{-1}$};
\node at (1, -0.2) {$z^{-1}$};
\node at (1.5, 1.3) {$u^{-1}$};
\node at (0.5, 1.3) {$v^{-1}$};
\draw[thick, -latex] (3.5,1)--(7,1);
\node at(5.2, 1.2)  {cluster~ mutations};
\end{tikzpicture}
\begin{tikzpicture}[scale=0.9]
\node at (0,0) {$\bullet$};
\node at (2,0) {$\bullet$};
\node at (0,2) {$\bullet$};
\node at (2,2) {$\bullet$};
\draw (0,0)--(2,0)--(2,2)--(0,2)--cycle;
\draw[dashed] (0,0) --(2,2);
\draw (2,0)--(0,2);
\node at (-0.2, 1) {$\tau(w)$};
\node at (1, 2.2) {$\tau(x)$};
\node at (2.2, 1) {$\tau(y)$};
\node at (1, -0.2) {$\tau(z)$};
\node at (1.5, 1.3) {$v$};
\node at (0.5, 1.3) {$u$};
\end{tikzpicture}
\end{center}
Here
\[
\tau(u)=v;  \hskip 14mm \tau(v)=u.
\]
\[
\tau(w)=w^{-1}(1+v^{-1})(1+u^{-1}); \hskip 14mm \tau(y)=y^{-1}(1+v^{-1})(1+u^{-1}); 
\]
\[
\tau(x)=x^{-1}(1+v)^{-1}(1+u)^{-1}; \hskip 14mm \tau(z)=z^{-1}(1+v)^{-1}(1+u)^{-1}; 
\]
Note that the mapping class group of punctured sphere acts on $\mathcal{P}$ by symplectomorphisms. The mapping class group preserves $\cM$, but it interchanges the other components of $\cM_i$.

In general, $\cM$ in Theorem \ref{thm:comparison} is a connected component of $\cM_i$. Therefore Theorem \ref{thm:comparison} is a special case of Theorem \ref{thm:general.lagrangian}.

%For general surfaces, we get many Lagrangians which depend on the reflection $i$ chosen.
\end{example}




% \section{Phases, Framings, Open Gromov-Witten Invariants and Mutation}
% \label{sec:pfogwiam}

% In \cite{TZ}, OGW framings were defined to generalize the notions of phase and framing used by \cite{AV, AKV} and many others to deduce
% enumerative geometry of Lagrangians in toric Calabi-Yau threefolds.  Framing is a term borrowed from knots in Chern-Simons theory, which
% is a large-N dual description of conormal branes in the resolved conifold --- see \cite{DSV} and \cite{AENV}, for example.
% We review the definition here and show how OGW framings (hereafter simply ``framings'') are transported across mutations.

% Recall that we consider a Legendrian surface $S_\Gamma\subset \bC^3$ defined by a cubic planar graph $\Gamma.$
% Lagrangian fillings of $S_{\Gamma}$ are associated with \emph{foams} $\bF \subset D^3$ \cite[Def. 3.1]{TZ} that fill the graph $\Gamma \subset \partial D^3$.
% If $\bF^1$ denotes the $1$-skeleton of $\bF$, then by smoothing out the vertices of $\bF^1$ we obtain \cite[\S 3.4]{TZ} a tangle $\cT$ --- there are as many as $3^k$ ways of doing this, where $k = \# \bF^0$ is the number of point-singularities of $\bF$.  The branched double cover of this tangle, called $L(\cT)$, admits a Lagrangian immersion (we hope it can be taken to be an embedding though we have not proved this) into $\bC^3$ that is asymptotic to $S_{\Gamma}$ \cite[\S 3.5]{TZ}.  We call $L(\cT)$ a \emph{phase} for $S_{\Gamma}$.\footnote{The terminology is motivated by the special case when $\Gamma$ is the tetrahedron graph.  Then $S_{\Gamma}$ is the boundary of three families of Harvey-Lawson Lagrangians in $\bC^3$, which Aganagic, Klemm and Vafa called ``phases'' of the Lagrangian brane in the open Gromov-Witten problem \cite{AV,AKV}.}

% \begin{example}[A foam filling for $\necklace_g$]
% \label{ex:foam-necklace}
% The necklace graph has a distinguished foam filling, that we in fact believe to be unique.  This foam has no vertices, so that $\bF^1$ is already smooth --- in other words there is a unique phase.  See Figure \ref{fig:necklacefoam} below.
% \begin{center}
% \begin{figure}[H]
% \begin{tikzpicture}
% %\draw[thick] (0,0) circle (2cm);
% \shadedraw[white,shading=ball,opacity=0.4] (0,0) circle (2cm);
% \draw[red,thick] (0,-1.414) ellipse (1.414cm and .2cm);
% \draw[red,thick] (1.414,-1.414) arc (-45:45:2cm);
% \draw[red,thick] (-1.414,1.414) arc (135:225:2cm);
% \draw[black,thick] (1.414,1.414) arc (45:135:2cm);
% %\draw[black,thick] (0,-2) arc (-90:-45:2cm);
% \draw[black,thick] (-1.414,-1.414) arc (-135:-45:2cm);
% \node at (1.414,1.414) {$\red{\bullet}$};
% \node at (1.414,-1.414) {$\red{\bullet}$};
% \node at (-1.414,-1.414) {$\red{\bullet}$};
% \node at (-1.414,1.414) {$\red{\bullet}$};
% \draw[blue,very thick] (0,-.5) parabola (1.414,-1.414);
% \draw[blue,very thick] (0,-.5) parabola (-1.414,-1.414);
% \draw[yellow, very thick] (0,.5) parabola (.3,1.6);
% \draw[yellow, very thick] (0,.5) parabola (-.15,1.25);
% \draw[yellow, very thick] (0,.5) -- (0,-.5);
% \draw[yellow, very thick] (0,-.5) parabola (-.3,-1.6);
% \draw[yellow, very thick] (0,-.5) parabola (.15,-1.25);
% \draw[yellow, very thick] (.5,.6) parabola (.8,1.6);
% \draw[yellow, very thick] (.5,.6) parabola (.4,1.2);
% \draw[yellow, very thick] (.5,.6) -- (.5,-.6);
% \draw[yellow, very thick] (.5,-.6) parabola (.8,-1.25);
% \draw[yellow, very thick] (.5,-.6) parabola (.3,-1.6);
% \draw[yellow, very thick] (1,.97) parabola (1.2,1.5);
% \draw[yellow, very thick] (1,.97) parabola (.9,1.25);
% \draw[yellow, very thick] (1,.97) -- (1,-.97);
% \draw[yellow, very thick] (1,-.97) parabola (1.2,-1.3);
% \draw[yellow, very thick] (1,-.97) parabola (.9,-1.55);
% \draw[yellow, very thick] (1.414,1.414) -- (1.414,-1.414);
% \draw[yellow, very thick] (1.8,.8) -- (1.8,-.8);
% \draw[yellow, very thick] (-.5,.6) parabola (-.8,1.2);
% \draw[yellow, very thick] (-.5,.6) parabola (-.4,1.6);
% \draw[yellow, very thick] (-.5,.6) -- (-.5,-.6);
% \draw[yellow, very thick] (-.5,-.6) parabola (-.8,-1.6);
% \draw[yellow, very thick] (-.5,-.6) parabola (-.3,-1.25);
% \draw[yellow, very thick] (-1,.97) parabola (-1.2,1.3);
% \draw[yellow, very thick] (-1,.97) parabola (-.9,1.5);
% \draw[yellow, very thick] (-1,.97) -- (-1,-.97);
% \draw[yellow, very thick] (-1,-.97) parabola (-1.2,-1.5);
% \draw[yellow, very thick] (-1,-.97) parabola (-.9,-1.3);
% \draw[yellow, very thick] (-1.414,1.414) -- (-1.414,-1.414);
% \draw[yellow, very thick] (-1.8,.8) -- (-1.8,-.8);
% \draw[blue,very thick] (0,.5) parabola (1.414,1.414);
% \draw[blue,very thick] (0,.5) parabola (-1.414,1.414);
% \draw[red,thick] (0,1.414) ellipse (1.414cm and .2cm);
% \end{tikzpicture}
% \quad 
% \includegraphics[scale=.8]{dinofoam.png}
% \caption{The necklace graph ${\necklace_g}$ with $g=1$, pictured in red at left, is drawn on the surface of a sphere.
% The canonical tangle (phase) is shown in blue.  Some cross-sections of the associated foam are shown in yellow.
% On the right, something close to a foam for ${\necklace_{11}}$.}
% \label{fig:necklacefoam}
% \end{figure}
% \end{center}
% %
% %The symplectic lattice $\Lambda_1$ has generators $a$ (for the arc) and $b$ for the bigon,
% %chosen so that $(a,b)=1.$  Call $u$ and $v$ the corresponding $\bC$-valued coordinate.
% %Since $b$ connects one strand of the tangle to itself, it lies in the
% %kernel of the map from $H_1(S,\bZ)\to H_1(L(\cT),\bZ).$
% %Any transverse coordinate to $v$ has the form $u + pv$, so we can label the framings (splittings)
% %by a single integer $p.$
% It will be important for us to analyze this in some detail --- continued in Example \ref{ex:frame-necklace}.
% \end{example}

% A phase of $S_{\Gamma}$ gives a Lagrangian polarization of $\cP_{\Gamma}$, which is just the short exact sequence of tori
% \begin{equation}
% \label{eq:phase-polar}
% 1 \to H^1(L(\cT),\bC^*) \to \cP_{\Gamma} \to H_1(L(\cT),\bC^*) \to 1
% \end{equation}
% In \cite[\S 4.8]{TZ}, we called $H^1(L(\cT),\bC^*)$ by $T_L$, though we will search for better notation in this document.  A framing of this phase is the data of a Lagrangian splitting of \eqref{eq:phase-polar}, which can be used to give a symplectic morphism (in fact a covering space map) 
% \[
% T^* (H^1(L(\cT),\bC^*)) \to \cP_{\Gamma},
% \]
% along which we can take the inverse image of the Lagrangian $\cM_{\Gamma}$.  On general grounds, this inverse image is the graph \red{(Why a graph?)} of a closed one-form, thus there is a (multiple-valued, transcendental) holomorphic function
% \[
% W_{\Gamma}:H^1(L(\cT),\bC^*) \to \bC
% \]
% such that the graph of $dW_{\Gamma}$ coincides with the pullback of $\cM_{\Gamma}$.  Some examples were computed in \cite[\S 5]{TZ}, where $W_{\Gamma}$ was found
% to be expressed as an integer combination of dilogarithms in every case, generalizing the observations of Aganagic-Klemm-Vafa on the Harvey-Lawson Lagrangians. 

% \begin{example}[Framings of the unique foam filling of $\necklace_g$]
% \label{ex:frame-necklace}
% The graph $\necklace_g$ with its canonical foam $\bF$ and unique phase also has a distinguished framing, i.e.~splitting, which we now describe.  
% In this case $\bF^1$ is nonsingular and its tangle $\cT$ is $g+1$ unlinked strands, each one connecting the two vertices
% of a single bead of the necklace.
% Let
% us label the beads of the necklace $0, 1, ..., g$ and call $u_i$, $i = 1,...,g$, the edge connecting bead $i-1$ to bead $i.$
% Note each $u_i$ connects different strands and together they generate $H_1(L(\cT)).$
% Let $v_i$, $i=1,...,g$, be the inner edge of bead $i$.  Then as $v_i$ connects a strand to itself it lies in the kernel of the 
% map $\cP \to H_1(L(\cT))$.  

% We define $x_i = \exp(u_i)$, a coordinate on $T_L$, which together with the $v_i $ coordinatize $T^*T_L$ (we sometimes put $y_i = \exp(v_i)$).
% They define a canonical framing for $\necklace$.  

% Having fixed the bases $u_i$ for $H_1(L(\cT))$ and $v_i$ for $H^1(L(\cT))$, we can parametrize all other framings by
% $g\times g$ integer-valued matrices $A$, so that the lift $\widetilde{e}_i$ of $u_i$ under $A$ is written as $u_i + A_{i,k}v_k.$  
% The requirement $(\widetilde{e}_i,\widetilde{e}_j) = 0$ implies $A_{i,j} - A_{j,i}=0,$ so $A$ is symmetric.
% \end{example}

% The main point of this section is the following theorem, which demonstrates
% that the above example suffices to study all framings, since they can be transported across mutations.

% \begin{theorem}
% Let $\Gamma$ be a cubic planar graph such that $S_\Gamma$ has genus $g$.
% Then framings of $\Gamma$ are canonically in 1-1 correspondence with framings of $\necklace_g$.
% Framings with a fixed phase are labeled by symmetric $g\times g$ matrices.
% \end{theorem}
% \begin{proof}
% \red{Isomorphisms $\nu$ are symplectic, so take framings to framings.  Hopefully, they are independent
% of the sequence of mutations from $\necklace_g$ to $\Gamma.$  Then connectivity of the graph of ideal triangulations.}
% \end{proof}

==> chromatic-lagrangian-and-wavefunction.tex <==

\subsection{Ekholm-Shende's wave function}

We consider the Aganagic-Vafa brane $L$ in $\C^3$. The Wave function defined by Ekholm-Shende is 
$$
\Psi_L = \sum_{u} (q^{1/2} - q^{-1/2})^{-\chi (u)} a^{u*L} \partial u,  
$$
where the sum is taking over all J-holomorphic disks with boundary in $L$, and $u*L$ is the linking number of $u$ and $L$, defined in their paper (and claimed to be related to the framing). This wave function lives in the completion of skein module $Sk(L)$. 

By analyzing the moduli space of J-holomorphic curves (which may not be very rigorous), they get equation:
$$
(\bigcirc - P_{1,0} + a \gamma P_{0,1}) \Psi = 0.
$$
where $\gamma$ is just some power of $a$. (and in the paper they have the notation $a_L$, which I think is just $a$.) Solving this equation we get:
$$
\Psi = \sum_{\lambda}  W_\lambda (\gamma^{|\lambda|} \prod_{\Box\in \lambda} \frac{q^{-c(\Box)/2}}{q^{h(\Box)/2}-q^{-h(\Box)/2} } )
$$
If we let $\gamma = 1$, this matches with the topological vertex with zero framing. But for different framing, we meet the first problem here:
\begin{q}
$\gamma$ is a power of $a$, which becomes a power of $q$ if we choose a specialization. Under a change of framing, the difference is a power of q, linear with respect to $|\lambda|$. However, according to topological vertex it should be quadratic. For example, in the rank $1$ case if a framing gives $\gamma = q^p $, then the E-S wave function differs by $p |\lambda|$ instead of $p |\lambda|^2$. So there's something weird here. 
\end{q}

\subsection{Constructible sheaves and chromatic lagrangian}
We try to relate the wave function to the chromatic lagrangian, obtained from the moduli of some constructible sheaves, as in the rank one case. 

We consider the Legendrian weave living in $T^\infty S^2$, given by the tetrahedron graph $\Gamma$. Denote by $Sh^2_{S_\Gamma} (\R^3) $ the constructible sheaves in $\R^3$ with microlocal rank 2, and with singular support in $S_\Gamma$. We have the microlocal monodromy functor: 
$$
\mu: Sh^2_{S_\Gamma} (\R^3) \longrightarrow Loc_{GL_2} (S_\Gamma) 
$$


\begin{equation*}
    \input{fig1.tikz}
\end{equation*}


The image is the chromatic Lagrangian $\mathcal{M}_\Gamma$. We denote by $m_i \in GL_2, i = 1, 2, 3$ the 3 monodromies along the three loops corresponding to three edges on $\Gamma$. Since $S_\Gamma$ is a torus, these are just A, B and A+B monodromies of the torus.  As in the rank 1 case $\mathcal{M}_\Gamma$ is given by the equations: 
\begin{align}
    &m_1 m_2 m_3 =1 \label{a}\\ 
    &  1 + m_1 + m_1m_2 =0 \label{b}
\end{align}

Now we consider a cluster chart of $Loc_{GL_2}(T^2)$ and try to find out what the chromatic Lagriangian $\mathcal{M}_L$ looks like in it. As Gus mentioned in the previous email we should first look at local systems on the punctured torus $Loc_{PGL_2} (T^2 \backslash pt)$. Let $x_1, x_2, x_3$ be the cluster variables. According to Frederic Palesi's note, we can calculate the monodromies explicitly. The monodromy around the puncture is
$$
\begin{pmatrix}
  (x_1x_2x_3)^2 & 0 \\
  (1 + x_1 x_2 x_3)(1 + x_3 + x_1 x_3) & 1
\end{pmatrix}
$$
We would like to ask $x_1x_2x_3 = -1$, so that the local system can extend to the non-punctured torus. 

A similar calculation shows that if we start from a point $p$, as is illustrated in the picture, the three $GL_2$ monodromies are:
$$
m_1 = -
\begin{pmatrix}
    x_1x_3 & x_1 x_3\\
    x_3 & 1 + x_3
\end{pmatrix};
m_2 = 
\begin{pmatrix}
    -1 - x_2 - x_2x_3 & -1 \\
    x_2x_3 & 0
\end{pmatrix};
m_3 = 
\begin{pmatrix}
    1 & -x_1\\
    -1 & x_1 + x_1 x_2
\end{pmatrix}
$$
They satisfy the equation (\ref{a}) and (\ref{b})



\begin{equation*}
    \input{p2.tikz}
\end{equation*}


A silly question is 
\begin{q}
    how to explicitly write down a cluster chart on $Loc_{GL_2}(T^2)$ ? (Since we know the $PGL_2$ case.)
\end{q} 
The method we use is taking the covering map:
$$
Loc_{GL_2}(T^2) \stackrel{det \times proj}{\longrightarrow} Loc_{\C^*}(T^2) \times Loc_{PGL_2}(T^2)
$$
and consider the image. Denote the coordinates on $Loc_{PGL_2}(T^2) $ by $a_1 = x_1$, $b_1 = x_2$, and coordinates on $Loc_{\C^*} (T^2)$ by $a = det \ m_1$ and $b = det \ m_2$. 

The equation for the image of the chromatic lagrangian is 
$$
ab_1 - 1 = 0; \ \ \ a_1 b + 1 = 0 .
$$

If we then do the naive quantization, we get the equations:

$$
(UV_1 +1) \Psi =0; \ \ \ (U_1V + 1) \Psi =0
$$
which doesn't seem correct...
This cannot match with E-S wave function, or the equations Gus derived...
\\

Also, I noticed in Gus's notes, he had the equation:
$$
(q^{\frac{1}{2}} + q^{-\frac{1}{2}} - M_1 + a\gamma(X_1, X_2) ) \Psi(X_1, X_2) =0. 
$$
and then he mentioned that $M_1$ and $X_1 + X_2$ are the quantum traces of holonomies around the A and B cycles of the torus. I got kind of confused here. Could you explain a little bit more or give some reference? 




==> qdl.tex <==

\section{Basics of compact $q$-dilogarithm}


Consider algebra $\mathcal{A}$ generated over $\mathbb{Z}[q^{\pm1}]$ by $U, V$ with relation $VU=q^2UV$. If $f\in\mathbb{Q}((q))[[z]]$ is a formal power series and $a$ an element of $\mathcal{A}$, then $f(a)$ makes sense as an element of the natural completion of $\mathcal{A}$.  

\begin{lemma}
There is exactly one non-constant formal series $\Psi\in\mathbb{Q}((q))[[z]]$ such that the following pentagon identity holds:
\begin{align}
\label{eq:penta}
\Psi(V)\Psi(U) = \Psi(U)\Psi(qVU)\Psi(V)
\end{align}
\end{lemma}
\begin{proof}
First note that by degree in $U,V$ considerations the `constant term' $c_0(q)$ in the expansion $\Psi = \sum_{n\geq0}c_n(q)z^n$ must be nonzero, and that by degree in $\Psi$ considerations this constant term must be $c_0(q)=1$. In particular, $\Psi(V)$ invertible in the completed algebra, and~\eqref{eq:penta} implies
\begin{align}
\label{eq:conj}
\Psi(V)\Psi(U)\Psi(V)^{-1} = \Psi(U)\Psi(qVU).
\end{align}
Comparing coefficients of $U$ in this equality, we get that
$$
\Psi(V)U\Psi(V)^{-1} = U+qVU.
$$
Inserting this back into the original pentagon identity~\eqref{eq:penta}
we see that any solution $\Psi$ must also satisfy the functional equation of the $q$-exponential:
\begin{align}
\label{eq:q-exp}
\Psi(U+qVU) = \Psi(U)\Psi(qVU).
\end{align}
By the same argument as in the $q=1$ case, this functional equation determines the power series $\Psi(z)=1+O(z)$ up to a rescaling $z\mapsto \lambda z$. Indeed, 
recalling the $q$-numbers $[m]_{q^2} =\frac{1-q^{2m}}{1-q^2}$, the $q$-binomial coefficients
$$
\binom{n}{k}_{q^2} = \frac{[n]_{q^2}}{[k]_{q^2}[n-k]_{q^2}}
$$
and $q$-binomial theorem 
$$
YX = q^2XY \implies \left(X+Y\right)^n = \sum_{k=0}^n\binom{n}{k}_{q^2}X^{n-k}Y^k,
$$
the functional equation~\eqref{eq:q-exp} is equivalent to the requirement that for all $n,k$ we have
\begin{align*}
c_nc_k = \frac{[n]_{q^2}}{[k]_{q^2}[n-k]_{q^2}}c_{n+k},
\end{align*}
so that $a_n := c_n/[n]!_{q^2}$ satisfy $a_na_k=a_{n+k}$, whence $c_n = c_1^n$.
But comparing the coefficient of $UV$ in~\eqref{eq:penta} we get that
$$
q^2 c_1^2 = c_1^2+ qc_1,
$$
and so either $c_1=0$ (in which case $c_n=c_1^n=0$ for all $n$, and $\Psi$ is constant) or 
$$
c_1 = \frac{1}{q-q^{-1}}.
$$
Thus the only possible non-constant solution of ~\eqref{eq:penta} is 
\begin{align}
\label{eq:qdl}
\Psi = \sum_{n\geq0}\frac{q^nz ^n}{\prod_{k=1}^n(q^{2k}-1)}.
\end{align}
It remains to show this series actually satisfies~\eqref{eq:penta}. But it is easy to see from~\eqref{eq:qdl} that 
$$
\Psi(q^2z) =(1+qz)\Psi(z),
$$ 
and this implies~\eqref{eq:conj}, which together with~\eqref{eq:q-exp} implies~\eqref{eq:penta}.
\end{proof}

%\section{Standard complex}
%Let us recall the construction of the standard complex that computes the cohomology of a group $G$. Let $\Oc = \Oc(G)$. It is an algebra in $\Rep(G)$, where we consider the action of $G$ on functions by
%$$
%(h\cdot \phi)(g) = \phi(h^{-1}g).
%$$
%Consider the complex
%\beq
%\label{prequotient-complex}
%\Oc\rightarrow \Oc^{\otimes2}\rightarrow \Oc^{\otimes3}\rightarrow\cdots,
%\eeq
%where the face map $\partial^{(n)}_i$ is the morphism of algebras (in $\Rep(G)$) that trivially embeds $\Oc^{\otimes n}$ into $\Oc^{\otimes(n+1)}$ using all but the $i$--th tensor factor, and the differential is
%$$
%d^{(n)} = \sum_{i=0}^n (-1)^i\partial^{(n)}_i.
%$$
%There is an isomorphism
%\begin{align*}
%\Oc^{\otimes n}&\longrightarrow\hr{\Oc^{\otimes(n+1)}}^G \\
%f(g_1,\ldots, g_n)\longmapsto &F(g_0,\ldots, g_n):=f(g_0^{-1}g_1,g_1^{-1}g_2,\ldots,g_{n-1}^{-1}g_n)
%\end{align*}
%whose inverse sends
%$$
%F(g_0,\ldots, g_n) \mapsto f(g_1,\ldots, g_n) = F(1,g_1,g_1g_2,g_1g_2g_3,~\ldots,~ g_1\cdots g_n).
%$$
%So taking invariants in~\eqref{prequotient-complex}, we get a complex
%\beq
%k\rightarrow \Oc\rightarrow \Oc^{\otimes2}\rightarrow\cdots
%\eeq
%with the induced differential 
%$$
%d^{(n+1)}_G : \Oc^{\otimes n}\rightarrow \Oc^{\otimes{n+1}}
%$$
%\begin{align}
%\label{std-diff}
%(d^{(n+1)}_G f)(g_1,\ldots, g_{n+1}) = f(g_2,\ldots, g_{n+1}) + \sum_{i=1}^{n-1}f(g_1,\ldots,g_{i}g_{i+1},\ldots, g_{n+1}) +f(g_1,\ldots, g_n).
%\end{align}
%When $G$ is e.g. a finite group, this complex is (a shift of) the one that computes the group cohomology $H^*(G,k)$ with coefficients in the trivial representation $k$.


%\section{The quantum setup}
%Let us write $R = \sum \alpha_i\otimes \xi^i$ for the $R$-matrix of $U_q(\mathfrak{g})$, which satisfies
%$$
%R \Delta R^{-1} = \Delta^{\mathrm{op}},
%$$
%as well as $R^{-1} = (S\otimes 1)(R), R = (S\otimes S)(R)$.
%Consider the algebra of quantum matrix coefficients $\Oc_q(G)$ and its subalgebra $A = \Oc_q(G/N)$.  We define the product in $\Oc_q(G)$ by 
%$$
%(\phi \star \psi)(x) = \sum_{i}\phi(\alpha_ix_1)\psi(\xi^ix_2), \qquad \phi,\psi\in \Oc_q(G), x\in U_q(\mathfrak{g}).
%$$
%This multiplication makes $\Oc_q(G)$ into an algebra object in the (braided) tensor category $\Rep_q(G\times G)$, with the action being given by
%$$
%\hr{x\boxtimes y\cdot \phi}(z) = \phi(Sx\cdot z\cdot y), \quad x,y,z\in U_q(\mathfrak{g}).
%$$
%%{\bf Question: is it a commutative algebra there? }
%%In fact, its subalgebra $A$ is a {\em commutative} algebra in $\Rep_q(G\times \overline{T})$.
% Note also that the antipode of $\Oq(G)$ defines an algebra \emph{automorphism} (!)
%$$
%S: (\Oq(G),\star)\rightarrow (\Oq(G),\star).
%$$
%
%
%Consider the algebra $\Oc_n:= \Oc_q(G)^{\bt n}$ in $\Rep_q(G)$, where the tensor products are braided with respect to the braiding on the left $G$-factor only. 
%%Consider the algebra $\Oc_n:= \Oc_q(G)^{\bt n}$ in $\Rep_q(G\times\overline{T}^n)$, where the tensor products are braided with respect to the braiding on the left $G$-factor only. 
%%Consider the algebra $\Oc_n:= \Oc_q(G)^{\bt n}$, where we define the algebra structure using the monoidal structure from $\mathrm{Vect}$; in particular $\Oc_n$ is \emph{not} an algebra object in $\Rep_q(G)$. {\bf Should we be working with braided tensor products?}
%Once again, we have face maps
%$$
%\partial_i : \Oc_n\rightarrow \Oc_{n+1}, \quad 1\leq i\leq n,
%$$
%which are maps of algebras in $\Rep_q(G)$.
%Let us introduce the shorthands
%\begin{align*}
%\tilde\Delta &= (S^{-1}\otimes 1)\circ\Delta,\\
%\overline\Delta &= (1\otimes S^{-1})\circ\Delta.
%\end{align*}
%If $M$ is a $\mathcal{O}_q(G)$-comodule (i.e. integrable $U_q(\mathfrak{g})$-module) write $M^G$ for its invariants. 
%\begin{lemma}
%There is an isomorphism of algebras 
%\begin{align*}
%\mathcal{I}_n:=(1\otimes m^{\otimes n}\otimes 1)\circ \tilde\Delta^{\otimes n}~:~\Oc_n &\rightarrow \hr{\Oc_{n+1}}^G.
%\end{align*}
%\end{lemma}
%%given by
%\begin{proof}
%For $n=1$, one easily checks that
%$$
%\tilde\Delta ~:~ \phi \mapsto S^{-1}\phi_1~\bt~ \phi_2.
%$$
%is an algebra isomorphism of $\Oq(G)$ onto the $G$-invariants in $\Oq(G)\bt\Oq(G)$. The statement for $n>1$ follows by induction and the functoriality of the braided tensor product of algebras. For instance when $n=2$, we have a pair of algebra maps $\tilde\Delta_{i} = \partial_i\circ\tilde\Delta$, and their tensor product
%$\tilde\Delta_1\bt\tilde\Delta_2:\Oc_2\rightarrow\Oc_3$ coincides with the desired map. 
%\end{proof}
%The inverse of this map factors as
%$$
%\mathcal{I}_n^{-1} = S^{\otimes n}\circ m_{0,1}\circ\hr{m_{1,2}\circ\overline{\Delta}_2}\circ\cdots \circ\hr{m_{n-2,n-1}\circ\overline{\Delta}_{n-1}}\circ\hr{m_{n-1,n}\circ\overline{\Delta}_n}
%$$
%
%Let us now see how the face maps are realized at the level of $G$-invariants by computing
%$$
%\partial^n_{G,i} : = \mathcal{I}_n^{-1}\circ\partial^n_i\circ\mathcal{I}_n.
%$$
%In complete analogy with the commutative case, they are nothing but
%\begin{align*}
%\partial^n_{G,0}(\phi^{(1)}\bt\cdots\bt\phi^{(n)}) &= 1\bt\phi^{(1)}\bt\cdots\bt\phi^{(n)},\\
%\partial^n_{G,n+1}(\phi^{(1)}\bt\cdots\bt\phi^{(n)}) &= \phi^{(1)}\bt\cdots\bt\phi^{(n)}\bt 1,\\
%\partial^n_{G,i}(\phi^{(1)}\bt\cdots\bt\phi^{(n)}) &= \Delta_i, \quad 1\leq i\leq n.
%\end{align*}

%\section{The pentagon and the quantum dilogarithm as an associator}
%As a warmup, we begin with the case $n=2$.  Let us determine the conditions on an invertible element of $F\in\Oc^2$ 
%such that the twist of the coproduct $\Delta:\Oc\rightarrow\Oc\bt\Oc$ $$
%\Delta^F = F \cdot \Delta
%$$
%remains coassociative. The needed condition is that
%$$
%\Delta_1(F) = F_{12}^{-1}F_{23} \Delta_2(F),
%$$
%i.e. that
%$$
%\partial_{G,3}(F)\star\partial_{G,1}(F) = \partial_{G,0}(F)\star\partial_{G,2}(F).
%$$
%On the other hand, if there exists some element $f\in\Oc$ such that
%$$
%F = (f\otimes f)^{-1}\Delta(f) = \partial_{G,2}(F)^{-1}\star\partial_{G,0}(F)^{-1}\star\partial_{G,1}(F),
%$$
%then the map $\Oc\rightarrow\Oc$ given by multiplication by $f$ is
%an isomorphism of coalgebras.
%{\bf Problem: I think this uses the wrong algebra structure...)}
%
%We now focus on the case $n=3$. Consider the monoidal category $\mathcal{C}$ of $\Oc$--comodules. {\bf (!!!)} Is there a nontrivial associator? Does understanding the equivalence of this with the standard category with trivial associator help us understand the $d^2=0$ issue? {\bf (!!!)}
%
% The monoidal structure is determined by the coproduct $\Delta:\Oc\rightarrow\Oc\bt\Oc$, and the associators are the trivial ones. Consider the problem of when the action of invertible element $\alpha\in\Oc_3$ defines an associator 
%$$
%\alpha :L\otimes M\otimes N \rightarrow L\otimes M\otimes N.
%$$

%
%\section{Pentagon}
%Consider the quantized algebra of functions algebra on the moduli space of local systems with pinnings on the 4-gon. It coincides with the $U_q(\mathfrak{g})$-invariants in the 4-fold braided tensor product $\Oq(G/N)^{\tilde\otimes n}$. It sits as a subalgebra inside the $U_q(\mathfrak{g})$-invariants in a braided tensor product of 4 copies of $\Oq(G)$, which we regard as a term in the quantum standard complex.  Consider the $G$-invariant element given by $\Psi(X_{0,1,2,3})$, where $X$ is the quantum cross-ratio (i.e. $\mathcal{X}$-coordinate). {\bf Issue: this is not a regular function}
%
%The face maps in the standard complex give maps from $\Oq((G/N)^4)$ to $\Oq((G/N)^5)$, the algebra associated to the 5-gon. Moreover, the images of the invariant $\Psi(X_{0,1,2,3})$ under these maps are the quantum dilogarithms coming from the mutations that make up the pentagon relation. 
%
%
%
%
%\section{Quantum Borel}
%Let $\mathcal{C}$ be the category of representations of some Hopf algebra $H$. Suppose there is an invertible element $\Psi$ in $H\otimes H$ such that for all $a\in H$ we have
%\beq
%\label{psi-conj}
%\Psi \Delta(a) = (a\otimes 1) \Psi.
%\eeq
%as well as the 5-term identity
%\beq
%\label{pentagon-id}
%\Psi_{12}\Psi_{23} = \Psi_{23}\Psi_{13}\Psi_{12}.
%\eeq
%Note that the property~\eqref{psi-conj} implies
%$$
%(\Delta\otimes1)(\Psi_{12}) =  \Psi_{12}^{-1}\Psi_{13}\Psi_{12}, \quad(1\otimes\Delta)(\Psi_{12}) =  \Psi_{23}^{-1}\Psi_{12}\Psi_{23}.
%$$
%Now consider the monoidal category $(\mathcal{C},\boxtimes)$, where $a\in H$ acts on $U\boxtimes V$ by $a\otimes 1\in H^{\otimes2}$. We equip it with the following nontrivial associator: if $U,V,W$ are objects of $\mathcal{C}$, then we define
%$$
%\alpha_{U,V,W} =\Psi_{V,W} : (U\boxtimes V)\boxtimes W \rightarrow U\boxtimes (V\boxtimes W).
%$$
%Let's check the pentagon identity. We have
%$$
%((V_1\boxtimes V_2)\boxtimes V_3)\boxtimes V_4\longrightarrow^{\Psi_{V_3,V_4}}(V_1\boxtimes V_2)\boxtimes (V_3\boxtimes V_4)\longrightarrow^{\Psi_{V_2,V_3\boxtimes V_4}}V_1\boxtimes (V_2\boxtimes (V_3\boxtimes V_4))
%$$
%while going the other way we get
%$$
%((V_1\boxtimes V_2)\boxtimes V_3)\boxtimes V_4\rightarrow^{\Psi_{V_2,V_3}}(V_1\boxtimes (V_2\boxtimes V_3))\boxtimes V_4\rightarrow^{\Psi_{V_2\boxtimes V_3,V_4}}V_1\boxtimes ((V_2\boxtimes V_3)\boxtimes V_4)\rightarrow^{\Psi_{V_3,V_4}}V_1\boxtimes (V_2\boxtimes (V_3\boxtimes V_4)).
%$$
%Note that $\Psi_{V_2,V_3\boxtimes V_4} = \Psi_{23}$ by definition of the $H$-action on $V_3\boxtimes V_4$, and similarly $\Psi_{V_2\boxtimes V_3,V_4}=\Psi_{24}$. Thus the pentagon axiom says that
%$$
%\Psi_{23}\Psi_{34} = \Psi_{34}\Psi_{24}\Psi_{23},
%$$
%which is exactly the identity~\eqref{pentagon-id}.
%
%Then we can use $\Psi$ to equip the identity functor $I:(\mathcal{C},\otimes)\rightarrow (\mathcal{C},\boxtimes)$ with the structure of a monoidal functor, with coherence map
%$$
%\Psi_{V,W}: I(V\otimes W) \rightarrow I(V) \boxtimes I(W).
%$$
%The fact that this indeed defines a monoidal functor follows again by the identity~\eqref{pentagon-id}.
%
%So the standard category of representations of the Hopf algebra (using coproduct to define the action on a tensor product, and with trivial associators) is equivalent to the category $(\mathcal{C},\boxtimes)$ where the tensor products are trivial but where there is an nontrivial associator given $\alpha_{U,V,W}$. 
%
%So a better way to tell this story might be the following: let's consider the monoidal category $(\mathcal{C},\boxtimes)$  with trivial tensor product \emph{and} trivial associator. Because the form of the coproduct is so simple, it's easy to identify what commutes with the diagonal action of $H$ on a triple tensor product -- it's just identified with $H^{\otimes2}!$ So we get to deform the associator by any element of $H\otimes H$ which satisfies~\eqref{pentagon-id}. But the right way to think of this element is as one of $H\otimes H\otimes H$ that happens to commute with the diagonal action. 
%
%On the other hand if we have an element $\Psi$ satisfying~\eqref{psi-conj}, then we can use it to identify precisely what is the commutant of the diagonal action in the standard category $(\mathcal{C},\otimes)$. 

%So we have a method of looking for deformations of the associator on $(\mathcal{C},\otimes)$:
%\begin{itemize}
%\item Find an element $\Psi$ satisfying~\eqref{psi-conj}; we don't actually require~\eqref{pentagon-id} for the purposes of this particular trick.
%\item Look for 3-cocycles of the form $\Psi_{23}^{-1}\Psi_{12}^{-1}\rho_{23}\Psi_{12}\Psi_{23}$.
%\end{itemize}
%We can do this for both $\mathcal{O}_q(G/N)$ and $\mathcal{O}_q(G)$, using triangles and squares respectively.


%Perhaps one take-away is that we should expect plenty of functions
%that commute with the diagonal action of $\Oq(G)$. 
%
%
%Also, even if this third cohomology is somehow well-defined, perhaps arbitrary classes don't correspond to deformations of the associator, just those that commute with the diagonal. 

%{\bf What would be nice to have: } An element in $\Oq(G)^{\otimes 3}$ which satisfies the 'face relations' and commutes with the diagonal action. That way we get a deformation of the associator on the category of $\Oq(G)^{\otimes 3}$ --modules. 
%
%{\bf Question: } How could one even hope to define cohomology groups? After all, the differential is surely not a group homomorphism...  

%We want to define an action of $\mathcal{C}$ on itself, i.e a functor
%$$
%\mathcal{C}\boxtimes\mathcal{C}\longrightarrow\mathcal{C}.
%$$
%which is associative up to some natural transformation.
%If $U,V$ are objects of $\mathcal{C}$, we define $U\triangleright V$ to be the vector space $U\otimes V$ where $a\in H$ acts by $a\otimes1$, i.e. just a direct sum of $\dim V$-copies of the representation $U$. The associator is the given by the isomorphism
%$$
%\Psi_{12} : (U_1\otimes U_2)\triangleright V \rightarrow U_1\triangleright(U_2\triangleright V).
%$$
%$$
%\phi\otimes\psi\otimes\rho\longmapsto S^{-1}\phi_{(1)}~\otimes~ \phi_{(2)}\star S^{-1}\psi_{(1)}~\otimes ~   \psi_{(2)}\star S^{-1} \rho_{(1)}~\otimes~ \rho_{(2)}.
%$$
%\begin{remark}
%This can be composed with any braiding of the tensor factors, since the $R$-matrix preserves the invariants. So maybe we can find a smart braid to compose with to make this an algebra map?
%\end{remark}
%Consider the complex in $\Rep_q(G\times\overline{T})$, where the tensor products are braided with respect to the braiding on the $G$-factor only.
%$$
%\Oc_q(G)\rightarrow \Oc_q(G)\tilde\otimes\Oc_q(G)\rightarrow\Oc_q(G)^{\tilde\otimes 3}\rightarrow\cdots
%$$ 

%\bibliographystyle{alpha}
%\begin{thebibliography}{FG06b}
%
%\bibitem[KN11]{KN11}
%Kashaev, Rinat M., and Tomoki Nakanishi. ``Classical and quantum dilogarithm identities.'' \emph{SIGMA. Symmetry, Integrability and Geometry: Methods and Applications} 7 (2011): 102.
%
%\bibitem[SS16]{SS16}
%{G.\,Schrader, A.\,Shapiro.}
%``A cluster realization of $U_q(\sl_\mathfrak{n})$ from quantum character varieties.''
%\emph{arXiv:1607.00271} (2016).
%
%
%\end{thebibliography}


==> references.tex <==

%Reference

\begin{thebibliography}{99}

\bibitem[ADKMV]{ADKMV} M. Aganagic, R. Dijkgraaf, A. Klemm, M. Mari\~no and C. Vafa,
\emph{Topological Strings and Integrable Hierarchies,} Commun.~Math.~Phys. {\bf 261} (2005) 451--516;
\href{https://arxiv.org/pdf/hep-th/0312085.pdf}{\tt arXiv:hep-th/0312085}.


\bibitem[AENV]{AENV} M. Agaganagic, T. Ekholm, L. Ng and C. Vafa,
\href{https://projecteuclid.org/journals/advances-in-theoretical-and-mathematical-physics/volume-18/issue-4/Topological-strings-D-model-and-knot-contact-homology/atmp/1415818564.full}{\emph{Topological Strings,
D-Model, and Knot Contact Homology}},
Adv. Theor. Math. Phys. {\bf 18} (2014) 827--956; 



%\bibitem[AGNT]{AGNT}
%I. Antoniadis, E. Gava, K. S. Narain and T. R. Taylor, \emph{Topological Amplitudes in
%String Theory,} Nucl. Phys. {\bf B413} (1994) 162--184.
%


\bibitem[AKV]{AKV} M. Agaganagic, A. Klemm and C. Vafa, \emph{Disk Instantons, Mirror Symmetry and the Duality Web,} Z. Naturforsch. {\bf A57} (2002) 1--28;
\href{https://arxiv.org/pdf/hep-th/0105045.pdf}{\tt arXiv:hep-th/0105045}.

%\bibitem[AMV]{AMV} M. Atiyah, J. Maldacena and C. Vafa, \emph{An M-Theory Flop as a Large $\cN$ Duality,} arXiv:hep-th/0011256.
%
\bibitem[AV]{AV} M. Aganagic and C. Vafa, \emph{Mirror symmetry, D-branes and counting holomorphic
di
scs,} 
\href{https://arxiv.org/pdf/hep-th/0012041.pdf}{\tt arXiv:hep-th/0012041}.

%
%\bibitem[AV2]{AV2} M. Aganagic and C. Vafa, \emph{Mirror symmetry and a $G_2$ Flop,} arXiv:hep-th/0105225.
%

% \red{
% \bibitem[A]{A} M.~Alim,
% \emph{Difference equation for the Gromov-Witten potential of the resolved conifold,}
% \href{https://arxiv.org/pdf/2011.12759.pdf}{\tt arXiv:2011.12759}.
% }

%\bibitem[AW]{AW} M. Atiyah and E. Witten, \emph{M-Theory Dynamics on a Manifold of $G_2$ Holonomy,} arXiv:hep-th/0107177.
%
\bibitem[BZ]{BZ} A. Berenstein and A. Zelevinsky. \emph{Quantum cluster algebras.} Adv. Math., 195(2): 405-455, 2005.
%
%\bibitem[B]{Birkhoff} G. Birkhoff, \emph{A determinant formula for the number of ways of coloring a map,} Ann. Math. (1912)
%
%\bibitem[BM]{BM} H. Brugesser and P. Mani, {Shellable decompositions of cells and spheres,} Math Scand {\bf 29} (1971) 197--205.

\bibitem[CZ]{CZ} R.~Casals and E.~Zaslow, \emph{Legendrian Weaves:  $N$-Graph Calculus, Flag Moduli and Applications,}
\href{https://arxiv.org/pdf/2007.04943.pdf}{\tt arXiv:math/2007.04943}; to appear in Geometry \& Topology.  %Geom.\&Topol.~{\bf xx}(2022) 111--111.

\bibitem[CCV]{CCV} S. Cecotti, C. C\'ordova, and C. Vafa,
\emph{Braids, walls, and mirrors,}
\href{https://arxiv.org/pdf/1110.2115.pdf}{\tt arXiv:1110.2115}.

%\bibitem[CNV]{CNV} S. Cecotti, A. Neitzke, and C. Vafa, \emph{R-Twisting and 4d/2d Correspondences,} arXiv:1006.3435.

\bibitem[CEHRV]{CEHRV} C. C\'ordova, S. Espahbodi, B. Haghighat, A. Rastogi, and C. Vafa, 
\emph{Tangles, generalized Reidemeister moves, and thre-dimensional mirror symmetry,} \href{https://arxiv.org/pdf/1211.3730.pdf}{\tt arXiv:1211.3730}.

\bibitem[D]{D} T.~Dimofte,
\href{https://projecteuclid.org/journals/advances-in-theoretical-and-mathematical-physics/volume-17/issue-3/Quantum-Riemann-surfaces-in-Chern-Simons-theory/atmp/1408562471.full}{\emph{Quantum Riemann Surfaces in Chern-Simons Theory}}, Adv.~Theor.~Math. Phys. {\bf 17} 479--599.
%;arXiv:1102.4847.

\bibitem[DGGo]{DGGo} T. Dimofte, M. Gabella and A. Goncharov,
\href{https://link.springer.com/article/10.1007/JHEP11(2016)151}{\emph{K-Deompositions and 3d Gauge Theories}}, 
J.~High Energ.~Phys. {\bf 2016}, 151 (2016).
%https://doi.org/10.1007/JHEP11(2016)151
%arXiv:1301.0192.

\bibitem[DGGu]{DGGu} T. Dimofte, D. Gaiotto, and S. Gukov, \emph{Gauge Theories Labeled by Three-Manifolds},
Commun. Math. Phys. {\bf 325} (2014) 367--417;
\href{https://arxiv.org/pdf/1108.4389.pdf}{\tt arXiv:1108.4389}.

\bibitem[DGH]{DGH}
T. Dimofte, S. Gukov, and L. Hollands, \emph{Vortex Counting and Lagrangian 3-manifolds,} Lett. Math. Phys. {\bf 98} (2011) 225--287;
\href{https://arxiv.org/pdf/1006.0977.pdf}{\tt arXiv:1006.0977}.




\bibitem[DSV]{DSV} D.-E. Diaconescu, V. Shende, and C. Vafa, {\em Large N duality, lagrangian cycles, and algebraic knots},
Comm. Math. Phys {\bf 319}.3 (2013), 813--863.

\bibitem[DWZ]{DWZ} H.~Derksen, J.~Weyman and A.~Zelevinsky, \emph{Quiver with potential and representations I:  Mutations,}
\href{https://arxiv.org/abs/0704.0649}{\tt arXiv:0704.0649}.

\bibitem[E]{E} A. I. Efimov,  \href{https://www.cambridge.org/core/services/aop-cambridge-core/content/view/00C640DAA72FBB1F88C546977284E396/S0010437X12000152a.pdf/cohomological-hall-algebra-of-a-symmetric-quiver.pdf}{\it Cohomological hall algebra of a symmetric quiver}, {Compositio Math}. 148(2012) 1136-1146. 


%\bibitem[E]{E} T. Ekholm, \emph{Morse flow trees and Legendrian contact homology in 1-jet spaces,} Geom. Topol. {\bf 11} (2007) 1083--1224.
%
%\bibitem[EHK]{EHK} T. Ekholm, K. Honda, and T. K\'alm\'an,
%\emph{Legendrian knots and exact Lagrangian Cobordisms,} 
%arXiv:1212.1519.

\bibitem[EKL]{EKL} T.~Ekholm, P.~Kucharski and P.~Longhi,
\emph{Physics and Geometry of Knots-Quivers Correspondence}, Commun.~Math.~Phys.~{\bf 379} (2020) 361--415;
\href{https://arxiv.org/pdf/1811.03110.pdf}{arXiv:1811.03110}.

\bibitem[ES]{ES} T.~Ekholm and V.~Shende,
\emph{Colored HOMFLYPT counts holomorphic curves,}
\href{http://arxiv.org/abs/2101.00619}{\tt arXiv:2101.00619}.

\bibitem[EL]{EL} S.~Evens and J.-H. Lu, \emph{Poisson geometry of the Grothendieck-Springer resolutions of a complex semisimple group.}
Mosc. Math. J. 7(4), 2007, 613-642. \href{https://arxiv.org/abs/math/0610123}{\tt arXiv:math/0610123}

\bibitem[F] {F} Faddeev, L. D. (2008). {\it Discrete series of representations for the modular double of the quantum group} $U_q(sl_2)$. Functional Analysis and Its Applications, 42(4), 330-335.




\bibitem[FG1]{FG1} V.V. Fock and A.B. Goncharov, {\it Moduli spaces of local systems and higher Teichmuller theory,} Publ. Math. IHES, n. 103 (2006) 1-212. \href{https://arxiv.org/abs/math/0311149}{\tt arXiv:math/0311149}

\bibitem[FG2]{FG2} V.V. Fock and A.B. Goncharov, {\it Cluster ensembles, quantization and the dilogarithm,}
\href{https://arxiv.org/pdf/math/0311245v7.pdf}{\tt arXiv:math/0311245v7}.

\bibitem[FG3]{FG3} V.V. Fock and A.B. Goncharov, {\it Dual Teichm\"uller and lamination spaces,} \href{https://arxiv.org/abs/math/0510312v1}{\tt arXiv:math/0510312v1}.


\bibitem[FKV]{FKV}
{L.\,Faddeev, R.\,Kashaev, A.\,Volkov.}
``Strongly Coupled Quantum Discrete Liouville Theory I: Algebraic Approach and Duality.'' \emph{Communications in Mathematical Physics} 219, no. 1 (2001): 199-219.


\bibitem[FL]{FL} B.~Fang and C.C.~M.~Liu,
\href{https://link.springer.com/content/pdf/10.1007/s00220-013-1771-5.pdf}{\emph{Open
Gromov-Witten Invariants of Toric Calabi-Yau 3-Folds}},
Commun.~Math.~Phys.~{\bf 323} (2013) 285--328.


\bibitem[FZ4]{FZ4} S. Fomin and A. Zelevinsky, {\it Cluster algebras IV: Coefficients.} {\it Compositio Mathematica,} 142:112-164, 2007.

\bibitem[Go]{Go} W.M. Goldman, \href{https://link.springer.com/content/pdf/10.1007/BF01389091.pdf}{\it Invariant functions on Lie groups and Hamiltonian flows of surface group representations}, Invent.~Math.~{\bf 85} (1986) 263--302.

\bibitem[G]{G} A.B.~Goncharov, {\it Ideal webs, moduli spaces of local systems, and 3d Calabi-Yau categories},
\href{https://arxiv.org/pdf/1607.05228v1.pdf}{\tt arXiv:1607.05228v1}.

\bibitem[GK]{GK} A.B. Goncharov and R. Kenyon, {\it Dimers and cluster integrable systems}, \href{https://arxiv.org/abs/1107.5588}{\tt arXiv:1107.5588}.

\bibitem[GS1]{GS1} A.B. Goncharov and L. Shen, {\it Donaldson-Thomas transformations of moduli spaces of G-local systems,} Adv. in Math., 327(2018), 225-348;  \href{https://arxiv.org/abs/1602.06479v2}{\tt arXiv:1602.06479}.


\bibitem[GS2]{GS2} A.B. Goncharov and L. Shen, {\it Quantum geometry of moduli spaces of local systems and representation theory,}
\href{https://arxiv.org/pdf/1904.10491.pdf}{\tt arXiv:1904.10491}.

%\bibitem[G]{G}H. Geiges, \emph{An Introduction to Contact Geometry,} Cambridge University Press (Cambridge) 2008.
%
%\bibitem[GKS]{GKS} S. Guillermou, M. Kashiwara, and P. Schapira,
%\emph{Sheaf Quantization of Hamiltonian Isotopies and
%Applications to Nondisplaceability Problems,} Duke Math J. {\bf 161} (2012): 201--245.

\bibitem[GHM]{GHM} A.~Grassi, Y.~Hatsuda, and M~Mari\~{n}o,
\href{https://link.springer.com/content/pdf/10.1007/s00023-016-0479-4.pdf}{\emph{Topological Strings
from Quantum Mechanics}}, Ann.~Henri Poincar\'e {\bf 17} (2016) 3177--3235.




\bibitem[GS]{GS} S.~Gukov and P.~Su\l{}kowski,
\href{https://link.springer.com/article/10.1007/JHEP02(2012)070}
{\emph{A-polynomial, B-model, and Quantization,}}
JHEP 1202 (2012) 070.
% \href{https://arxiv.org/pdf/1108.0002.pdf}{\tt arXiv:1108.0002}.



\bibitem[HM]{HM} J. Harvey and G. Moore, \emph{Algebras, BPS States and Strings,} Nucl. Phys. {\bf B463} (1996) 315--368.

%\bibitem[H]{H} M. Haskins, Special Lagrangian Cones....
%Haskins M, Kapouleas N, 2007, Special Lagrangian cones with higher genus links, INVENTIONES MATHEMATICAE, Vol: 167, Pages: 223-294
%

\bibitem[HRV]{HRV} T. Hausel and F. Rodriguez Villegas, with an appendix by N. Katz, \emph{Mixed Hodge polynomials of character
varieties,} Invent. Math. {\bf 174} (2008) 555-625.

\bibitem[HLRV]{HLRV} T.~Hausel, E.~Letellier and F.~Rodriguez Villegas,
\href{http://annals.math.princeton.edu/wp-content/uploads/annals-v177-n3-p08-s.pdf}
{\emph{Positivity for Kac polynomials and DT-invariants of quivers}},  Annals of Math. 177 (2013), 1147-1168. 

\bibitem[H]{H} J.~Hua,
\emph{A refinement of Kac polynomials for quivers with enough loops,}
\href{https://arxiv.org/pdf/2207.09839.pdf}{\tt arXiv:2207.09839}.

\bibitem[I]{I} V.~Iacovino, \emph{Open Gromov-Witten Invariants and Boundary States}, \href{https://arxiv.org/pdf/1807.08786.pdf}{\tt arXiv:1807.08786}.

\bibitem[IKV]{IKV} A.~Iqbal, C.~Koz\c{c}az and C.~Vafa,
\href{https://iopscience.iop.org/article/10.1088/1126-6708/2009/10/069/pdf}{\emph{The refined topological vertex}},
J.~High Energ.~Phys. {\bf 10} (2009) 069.

\bibitem[J]{J} X.~Jin, \href{https://projecteuclid.org/journals/geometry-and-topology/volume-19/issue-3/Holomorphic-Lagrangian-branes-correspond-to-perverse-sheaves/10.2140/gt.2015.19.1685.full}{\emph{Holomorphic Branes Correspond to Perverse Sheaves}},
Geometry \& Topology {\bf 19} (2015) 1685--1735.

%\bibitem[JT]{JT} X. Jin and D. Treumann, work in progress.

%\bibitem[J]{J} D. Joyce, \emph{On Counting Special Lagrangian Homology 3-Spheres,} hep-th/9907013.

%\bibitem[J]{J} D. Joyce, \emph{Special Lagrangian Submanifolds with Isolated Conical Singularities V:
%Survey and Applications,} Jour. Diff. Geom. {\bf 63} (2003) 279--347.

%\bibitem[J2]{Joyce2} D. Joyce, \emph{Special Lagrangian Submanifolds with Isolated Conical Singularities I:
%Regularity,}
%
%\bibitem[KL]{KL} S. Katz and C.-C. M. Liu,
%\emph{Enumerative Geometry of Stable Maps with Lagrangian Boundary Conditions and Multiple Covers of the Disc,}
%Adv. Theor. Math. Phys. {\bf 5} (2000) 1--49.
%
%\bibitem[KS]{KS} Masaki Kashiwara and Pierre Schapira, \emph{Sheaves on Manifolds,} 
%Grundlehren der Mathematischen Wissenschafte
%{\bf 292} (Springer-Verlag, 1990).

\bibitem[Ka]{Ka}
{R.\,Kashaev.}
``The Quantum Dilogarithm and Dehn Twists in Quantum Teichm\"uller Theory.''
\emph{Integrable Structures of Exactly Solvable Two-Dimensional Models of Quantum Field Theory} (2001): 211-221.


\bibitem[KL]{KL} S.~Katz and C.-C.~M.~Liu,
\href{https://www.intlpress.com/site/pub/files/_fulltext/journals/atmp/2001/0005/0001/ATMP-2001-0005-0001-a001.pdf}{\emph{Enumerative Geometry of Stable Maps with
Lagrangian Boundary Conditions and Multiple Covers of the Disc}},
Adv.~Theor.~Math.~Phys.~{\bf 5} (2001) 1--49.


\bibitem[K]{K} B.~Keller,
\href{https://webusers.imj-prg.fr/~bernhard.keller/publ/Keller-FPSAC-2013.pdf}{\emph{Quiver mutation and combinatorial DT-invariants}}.

\bibitem[KN]{KN}
Kashaev, Rinat M., and Tomoki Nakanishi. ``Classical and quantum dilogarithm identities.'' \emph{SIGMA. Symmetry, Integrability and Geometry: Methods and Applications} 7 (2011): 102.

\bibitem[KS]{KS} Kontsevich, Soibelman,
\href{http://intlpress.com/site/pub/files/_fulltext/journals/cntp/2011/0005/0002/CNTP-2011-0005-0002-a001.pdf}
{\it Cohomological Hall algebra, exponential Hodge structures and motivic Donaldson-Thomas invariants}, CNTP {\bf 5} (2011) 231--352.  %\bibitem[Khov]{Khovanov} M. Khovanov, ``$\mathfrak{sl}_3$ link homology''

\bibitem[KRSS]{KRSS} P.~Kucharski, M.~Reineke, M.~Sto\v{s}ic, and P.~Su\l{}kowski,
\emph{Knots-quivers correspondence,} Adv.~Theor.~Math.~Phys.~{bf 23} (2019) 1849--1902;
\href{https://arxiv.org/pdf/1707.04017.pdf}{arXiv:1707.04017}.

\bibitem[LMV]{LMV} J.~Labastida, M.~Mari\~no and C.~Vafa, \href{https://iopscience.iop.org/article/10.1088/1126-6708/2000/11/007/pdf}{\emph{Knots, links and branes at large $N$}}, 
J.~High Energ.~Phys. {\bf 2000}, 11 (2000).

\bibitem[Le]{Le} I.~Le, \href{https://www.cambridge.org/core/journals/forum-of-mathematics-sigma/article/cluster-structures-on-higher-teichmuller-spaces-for-classical-groups/D705F1B18EF0793A2D2CC8BFE5D6B336}{\emph Cluster structures on higher Teichmuller spaces for classical groups,} Forum of Math, Sigma {\bf 7} (2019). 

\bibitem[LZ]{LZ} W. Luo and S. Zhu, {\it Integrality structures in topological strings I:  framed unknot,} \href{https://arxiv.org/pdf/1611.06506.pdf}{\tt arXiv:1611.06506}.

\bibitem[N]{N} David Nadler, {\em Microlocal branes are constructible sheaves},
Selecta Math. (N.S.) {\bf 15} (2009) 563--619;
\href{https://arxiv.org/pdf/math/0612399.pdf}{\tt arXiv:math/0612399}.

%\bibitem[N2]{N-cone} D. Nadler, {\em A combinatorial calculation of the Landau-Ginzburg model $M= \mathbb C^3,$ $W=z_1 z_2 z_3$},
%arXiv:1507.08735.

\bibitem[NZ]{NZ} David Nadler and Eric Zaslow, 
\href{https://www.ams.org/journals/jams/2009-22-01/S0894-0347-08-00612-7/S0894-0347-08-00612-7.pdf}{{\em Constructible Sheaves and the Fukaya Category}}, J. Amer. Math. Soc. {\bf 22} (2009), 233--286.




\bibitem[NT]{NT} T.~Nakatsu and K.~Takasaki,
\emph{Open string amplitudes of closed topological vertex,}
J.~Phys.~A: Math.~Theor.~{\bf 49} (2016) 025201;
\href{https://arxiv.org/pdf/1507.07053.pdf}{\tt arXiv:1507.07053}.



%\bibitem[NRSSZ]{NRSSZ} Lenhard Ng, Daniel Rutherford, Vivek Shende, and Steven Sivek, 
%and Eric Zaslow, {\em Augmentations are Sheaves},  arXiv:1502.04939.
%
\bibitem[OV]{OV} H. Ooguri and C. Vafa, \emph{Knot invariants and topological strings,} Nucl.
Phys. {\bf B577} (2000) 419--438;
\href{https://arxiv.org/pdf/hep-th/9912123.pdf}{\tt arXiv:hep-th/9912123}.

%\bibitem[P]{P} Y. Pan, \emph{Exact Lagrangian Fillings of Legendrian $(2,n)$ Torus Knots,} {\tt arXiv:1607.03167.}

%\bibitem[R]{Rizell} G. Rizell, \emph{Knotted Legendrian surfaces with few Reeb chords}, Algebraic and Geometric Topology {\bf 11}, (2011).
%
\bibitem[RV]{RV} F. Rodriguez Villegas, \emph{A refinement of the $A$-polynomial of quivers,} \href{https://arXiv.org/abs/1102.5308}{\tt arXiv:1102.5308}.
.


%\bibitem[RS]{RS} D. Rutherford and M. Sullivan, \emph{Cellular Legendrian Contact Homology for Surfaces, Pari I,}
%arXiv:1608.02984,
%and
%\emph{Cellular Legendrian Contact Homology for Surfaces, Pari II,}
%arXiv:1608:03011.
%
%\bibitem[SS]{Nicolo} S. Scherotzke and N. Sibilla
%
\bibitem[S]{S} L. Shen, \emph{Duals of Semisimple Poisson–Lie Groups and Cluster Theory of Moduli Spaces of G-local Systems}, International Mathematics Research Notices, Volume 2022, Issue 18, September 2022, Pages 14295--14318, \url{https://doi.org/10.1093/imrn/rnab094}

\bibitem[ST]{ST} J. Solomon and S. Tukachinsky, \emph{Point-like Bounding Chains in Open Gromov-Witten Theory,}
Geom. \!Funct. \!Anal. \!{\bf 31} (2021) 1245--1320;
\href{https://arxiv.org/pdf/1608.02495.pdf}{\tt arXiv:1608.02495}.

\bibitem[STWZ]{STWZ} V. Shende, D. Treumann, H. Williams and E. Zaslow, \emph{Cluster Varities from Legendrian Knots,}
Duke Math. \!J. \!{\bf 168} (2019) 2801--2871;
\href{https://arxiv.org/pdf/1512.08942.pdf}{\tt arXiv:1512.08942}.
%
%\bibitem[STW]{STW} V. Shende, D. Treumann, and H. Williams,
%\emph{On the combinatorics of exact Lagrangian surfaces,}
%arXiv:1603.07449.
%
%\bibitem[STZ]{STZ} V. Shende, D. Treumann, and E. Zaslow, \emph{Legendrian knots and constructible sheaves,} arXiv:1402.0490.




\bibitem[T]{T} K.~Takasaki,
\emph{Remarks on partition functions of topological string theory on generalized conifolds,}
RIMS Kokyuroku No.~1913 (2014), 182--201;
\href{https://arxiv.org/pdf/1301.4548.pdf}{\tt arXiv:1301.4548}.




\bibitem[TZ]{TZ} D. Treumann and E. Zaslow,
\href{https://www.intlpress.com/site/pub/files/_fulltext/journals/atmp/2018/0022/0005/ATMP-2018-0022-0005-a005.pdf}{\emph{Cubic Planar Graphs and Legendrian Surface Theory}},
Adv. \!Theor. \!Math. \!Phys. \!{\bf 22} (2018) 1289--1345.

%\bibitem[Y]{Yau} M.-L. Yau, 
%\emph{Surgery and invariants of Lagrangian surfaces,} arXiv:1306.5304.

\bibitem[V]{V}
{A.Y.\,Volkov,}
\emph{Noncommutative hypergeometry},
Commun. \!Math. \!Phys. \!{\bf 258} (2005) 257--273;
\href{https://arxiv.org/pdf/math/0312084.pdf}{arXiv:math/0312084}.

\emph{Communications in mathematical physics} 258, no. 2 (2005): 257-273.


\bibitem[Z]{Z} D.~Zagier, {\emph{The Dilogarithm Function}},
in: Cartier P., Moussa P., Julia B., Vanhove P. (eds),
Frontiers in Number Theory, Physics, and Geometry II. Springer, Berlin, Heidelberg, 2007;
also available \href{https://people.mpim-bonn.mpg.de/zagier/files/doi/10.1007/978-3-540-30308-4_1/fulltext.pdf}{here}.

\bibitem[Za]{Za} E.~Zaslow,
\emph{Wavefunctions for a Class of Branes in Threespace},
\href{https://arxiv.org/pdf/1803.02462.pdf}{\tt arXiv:1803.02462}.


\end{thebibliography}



==> the-wavefunction-of-AV-brane.tex <==

\section{The Wavefunction of the AV brane}

\subsection{The Topological Vertex = ES}

The topological vertex wave function for the AV brane (with framing $p$) is given by
$$
\Psi^{(p)} (q;x ) = \sum_\lambda W_\lambda^{(p)}(q) s_\lambda(x)
$$
with 
$$
W_\lambda^{(p)} = q^{p \kappa_\lambda/2 + \kappa_\lambda/4} \prod_{\Box \in \lambda}  \frac{1}{q^{h(\Box)/2} - q^{-h(\Box)/2}}, 
$$
where $\kappa_\lambda \coloneqq \sum_i \lambda_i(\lambda_i- 2i +1)$, and $h(\Box)$ is the hook length. 
\\


On the other hand, the Ekholm-Shende wave function is
$$
\Psi = \sum_\lambda \Psi_\lambda Q_\lambda
$$ 
with 
$$
\Psi_\lambda = \gamma^{|\lambda|} \prod_{\Box \in \lambda} \frac{q^{-c(\Box)/2}}{q^{h(\Box)/2} - q^{-h(\Box)/2}},
$$
where $c(\Box) = coarm - coleg$. 
\\

Now we compare the two. They only differ by a power of $q$. 
\begin{align}
	\sum_{\Box \in \lambda} c(\Box) \notag
	& = \sum_i \sum_{k = 1}^{\lambda_i} k - i \notag \\
	& = \sum_i \frac{\lambda_i(\lambda_i-2i +1)}{2} \notag \\
	& = \frac{1}{2} \kappa_\lambda \label{c}
\end{align}

Thus if we choose $p=-1$ and $\gamma = 1$, the two wave function matches up. 

\subsection{Baxter operator and wavefunction}

Recall the topological vertex formula can be also written in the form:
$$
\Psi = \sum_\lambda s_\lambda(q^\rho) s_\lambda (x) ,
$$
where $q^\rho = (q^{-1/2}, q^{-3/2}, q^{-5/2}, ... )$, $x = (x_1, x_2, ...)$ and $s_\lambda$ are the Schur polynomials.

We can use the following Cauchy's identity:
$$
\sum_\lambda s_\lambda(x) s_\lambda(y) = \prod_{i, j \geq 0} \frac{1}{1-x_i y_j} = \e (\sum_d \frac{1}{d} p_d (x) p_d (y)).
$$
where $x = (x_1, x_2, ...), y_j = (y_1, y_2, ...)$ and $p_d$ is the dth power sum. 

Thus 
$$
\sum_\lambda s_\lambda(q^\rho) s_\lambda (x) = \prod_{i, j} \frac{1}{1- (q^\rho)_i x_j} = \e(\sum_k \frac{1}{k}p_k(q^\rho) p_k(x)) = \E( \frac{1}{q^{1/2} - q^{-1/2}} p_1(x)),
$$

\begin{comment}
	\textcolor{red}{But I got a sign issue here. According to Gus's notes page (0.9.2), $Q_{\mathbf{x}} (-z) = \E( \frac{-z}{q^{1/2}-q^{-1/2}} P_\mathbf{x})$. So we have $\Phi^{(0)} = (Q_{(0,1)}(-1) \cdot 1 )^{-1} $ . Maybe we should take $-z$ as line element? If that is the case, we have $Q_{(0,1)} (1)\cdot 1 = \Phi^{(0)}$ 	
		Or, we can check that if we work over the field $\C((q))$ instead of $\C((q^{-1}))$, $Q_{(0,1)} (1)\cdot 1 = \Phi^{(0)}$ also holds}.
	
	For a general framing $p$, I would guess $\Phi^{(p)} $ is given by $ Q_{(p, 1)} \cdot 1$? 
\end{comment}


According to Gus's note (0.9.2), the Baxter operators can be defined as $Q_\mathbf{x}(-z) = \E(\frac{-z}{q^{1/2} - q^{-1/2} }P_\x )$, where $P_\x$ lives in the skein algebra of $T^2$. So we get:
\begin{equation}
(Q_{0, 1}(-1) \cdot 1)^{-1} = \Psi^{(0)} \label{0}
\end{equation}

On the other hand, we have 
$$
   s_\lambda(q^{-\rho}) = (-1)^{|\lambda|}q^{-\frac{1}{4}\kappa_\lambda} s_\lambda (q^\rho) 
$$
We can express the framing $-1$ wavefunction as 
\begin{align}
	\Psi^{(-1)} &= \sum_\lambda q^{-\frac{1}{4} \kappa_\lambda} s_\lambda(q^\rho) s_\lambda(x) \notag\\
				&= \sum_\lambda s_\lambda(q^{-\rho}) s_\lambda(-x) \notag\\
				&= \e(\sum_m \frac{1}{m} \frac{1}{q^{-m/2} - q^{m/2}} p_m(-x) ) \notag \\				
				&= Q_{(0,1)} (1) \cdot 1\label{-1} \\
				&= \E ( \frac{1}{q^{1/2} - q^{-1/2}}p_1 - \frac{1}{q - q^{-1}} p_2)\notag
\end{align}


Now let's consider general framing. 
\begin{prop}
$$
\E(\frac{1}{q^{1/2} - q^{-1/2}} P_{(p,1)} ) = \Psi^{(p)}
$$
\end{prop}

\begin{proof}
Let $q^{\frac{p}{2}\kappa}$ to be the operator acting by multiplying  $q^{\frac{p}{2}\kappa_\lambda}$ on $W_\lambda$. 
\begin{align*}
	\Psi^{(p)}  &= q^{\frac{p}{2} \kappa } \cdot \Psi^{(0)} \\
	&= \Ad_{q^{\frac{p}{2} \kappa }} \E (\frac{1}{q^{1/2} - q^{-1/2}} P_{0,1} ) \cdot 1\\
	&= \e (\sum_n \frac{1}{n} \frac{1}{q^{n/2} - q^{-n/2}} \Ad_{q^{p\kappa/2}} (P_{0, n})) \cdot 1
\end{align*}

Thus we only need to show 
\begin{equation}
\Ad_{q^{p\kappa/2}} P_{(0,n)} = P_{(pn, n)} \label{ad}
\end{equation}

According to Morton-Samuelson Thm 4.3, LHS of \eqref{ad} acts by:
\begin{align*}
 \Ad_{q^{p\kappa/2}} P_{(0,n)} \cdot Q_\lambda  = \sum_{\alpha \in \lambda + n} q^{\frac{p}{2}(\kappa_\alpha - \kappa_\lambda)} (-1)^{ht(\alpha - \lambda)} Q_\alpha  ,
\end{align*}

while the RHS of \eqref{ad} acts by:
$$
 P_{(pn, n)} \cdot Q_\lambda = a^{pn} \frac{\{pn\}}{ \{pn^2\} } (\sum_{\alpha \in \lambda + n} (-1)^{ht(\alpha - \lambda) } C_{\alpha - \lambda} (q^{pn}) Q_\alpha  ).
$$

Here $\alpha \in \lambda + n$ means that $\alpha - \lambda$ is a ``border strip'' of size $n$, i.e. it is connected and contains no $2 \times 2$ squares, $\{n\} = q^{n/2} - q^{-n/2}$, and $C_{\alpha - \lambda} (t) = \sum_{\box \in  \alpha - \lambda } t^{c(\Box)}  $ . 

\textcolor{red}{We still have this $a$ here. Need to set $a$ to be 1 in order to make things match up..}

Take $a = 1$. Now, what's left to show is 
\begin{align*}
 C_{\alpha - \lambda}  (q^{pn}) = \frac{\{pn^2\}}{\{pn\}} q^{\frac{p}{2} (\kappa_\alpha - \kappa_\lambda)}
\end{align*}
We can assume $p = 1$, and use \eqref{c}. The above is equivalent to
\begin{align}
\sum_{\Box \in \alpha - \lambda} q^{n c(\Box)} 
= (q^{\frac{n}{2} (n-1 )} + q^{\frac{n}{2}(n-3) } + \cdots q^{- \frac{n}{2} (n-1) } ) q^{ \sum_{\Box \in \alpha - \lambda} c(\Box)} \label{border}
\end{align}
Since $\alpha - \lambda $ is a ``border strip'' of size $n$, if we denote the very lower-left box of this border strip by $\boxtimes$, we have
$$\sum_{\Box \in \alpha - \lambda} q^{n c(\Box)}  = q^{n c(\boxtimes)} + q^{n (c(\boxtimes) +1) } + q^{n (c(\boxtimes) +2) } + \cdots q^{n (c(\boxtimes) + n-1) }
$$
and
 $$
 \sum_{\Box \in \alpha - \lambda} c(\Box) = n c(\boxtimes) + \frac{n(n-1)}{2}. 
 $$ 
 
 Thus the two sides of \eqref{border} match up. 

\end{proof}

\subsection{Pentagon relation}
We want to show the pentagon relation for Baxter operators: 
\begin{equation}
	Q_{\x} Q_{\y} = Q_{\y} Q_{\x+\y} Q_{\x} 
\end{equation}
where $det\{\x, \y\} = 1$. 

First, let us compute $\Ad_{Q_\x} P_{\z}$, assuming $det\{\x, \z\} = d$.  Take $s = q^{1/2}$, and $\{k\} \coloneqq s^k - s^{-k}$. 

Set $\Theta_{\x} \coloneqq \sum_{k\geq1} \frac{(-1)^{k+1}}{k\{k\}} P_{k\x}$. Then $Q_\x = \e (\Theta_\x)$. We have:

$$
\ad_{\Theta_\x} P_\z = \sum_{k \geq 1} \frac{\{kd\}}{k\{k\}} (-1)^{k+1} P_{k \x + \y }
$$
and 
\begin{align*}
	\Ad_{Q_\x} \cdot P_\z 
	&= e^{\ad_{\Theta_\x}} \cdot P_\z \\
	&= \sum_n \frac{1}{n!} (\ad_{\Theta_\x})^n P_\z \\
	&= \sum_N \sum_{k_1 + \cdots +k_n = N} \frac{1}{n!} (-1)^{N+n} \prod_i \frac{\{k_i d\}}{k_i \{k_i\}} P_{N\x + \y}                
\end{align*}

Take 
$$c^{(d)}_N \coloneqq  \sum_{k_1 + \cdots +k_n = N} \frac{1}{n!} (-1)^{N+n} \prod_i \frac{\{k_i d\}}{k_i \{k_i\}}.
$$
As Gus indicated, these $c^{(d)}_N$ are q-bimonial coefficients. My way of seeing this is: 
\begin{align*}
	\sum_k \frac{\{kd\}}{k\{k\}} (-1)^{k+1} x^k
	&= \sum_k \frac{1}{k} (s^{(d-1)k } + s^{(d-3)k} + \cdots s^{-(d-1)k} ) (-1)^{k+1} x^k \\
	&= \l(1+ x s^{d-1}) + \cdots + \l(1+ x s^{-(d-1)})	
\end{align*}
Thus 
\begin{align*}
	f^{(d)} 
	&\coloneqq \sum_n c_n^{(d)} x^n \\
	&= \e(	\sum_k \frac{\{kd\}}{k\{k\}} (-1)^{k+1} x^k)\\
	&= (1 + xs^{d-1}) (1 + xs^{d-3} ) \cdots (1 + s^{-(d-1)})
\end{align*}
Similarly we can get:
\begin{align*}
	f^{(-d)} 
	&\coloneqq \sum_n c_n^{(-d)} x^n \\
	&= \frac{1}{(1 + xs^{d-1}) (1 + xs^{d-3} ) \cdots (1 + s^{-(d-1)})}
\end{align*}

\textcolor{red}{For $d>0$ we have $c_n^{(d)} = {d \choose n}_q = \frac{\{d\}!}{\{n\}! \{d-n\}!}$. (Note: might differ by some power of $q$ from the usual definition of q-binomial coefficients!) For $c_n^{(-d)}$ we have \eqref{x}}.

Now lets try to show 
\begin{equation}
	\Ad_{Q_\x} \Ad_{Q_\y} = \Ad_{Q_\y} \Ad_{Q_{\x +\y }} \Ad_{Q_\x} \label{ad2}
\end{equation}

If we consider the action on general $P_z$, I think \eqref{ad} boils down to 
$$
 c^{(b+M)}_N \cdot c_M^{(a+N)} = \sum_{l \in \mathbb{Z}} c_{(M-l)}^a \cdot c_l^{(a + b +l)} \cdot c_{N-l}^{(b)}
$$
But I've no clue how to show this. 

However, the algebra $\widehat{Sk(T^2)}$ is generated by $P_{\pm \x}, P_{\pm \y}$. So we only need to show that \eqref{ad} for these generators. 

$P_{-\x}$ and $P_{\y}$ are easy. 

Let us consider Case $P_\x$: 
\begin{align*}
	\Ad_{Q_\x} \Ad_{Q_\y} \cdot P_\x 
	& = \sum_{k\geq 0} (-1)^k \Ad_{Q_\x} P_{\x + k\y } \\
	& = \sum_{k\geq 0, l\geq 0} (-1)^k c_l^{(k)}P_{l\x + k \y + \x} ,
\end{align*}
while
\begin{align*}
	\Ad_{Q_\y} \Ad_{Q_{\x + \y}} \Ad_{Q_\x} \cdot P_\x  
	& = \Ad_{Q_\y} \Ad_{Q_{\x+\y}} P_\x\\
	& = \Ad_{Q_\y} \sum_{k\geq 0} P_{k\x  + k\y +\x}\\
	& = \sum_{k, l\geq 0} (-1)^k c_l^{(-(k+1))} P_{k\x + (k+l) \y +\x}
\end{align*}
Compare the coefficients of the term $P_{M\x + N\y + \x} $, we need to show:
\begin{equation*}
c_M^{(N)} = (-1)^{N-M} c_{N-M}^{(-N - 1)}, \ \ \ \text{for all}\  M, N \geq 0, 
\end{equation*}
which can be rewritten as
\begin{equation}
 (-1)^k	c_k^{(-(l+1))} = c_l^{(k+l) }  \label{x}
\end{equation}
\textcolor{red}{I guess this is some standard result? However I didn't find any reference...}
\begin{proof}[proof of \eqref{x}]

Take generating functions. Then \eqref{x} is equivalent to 
\begin{align}
f^{(l+1)} ( -x ) 
& = \frac{1}{(1- s^l x ) (1 - s^{(l-2)} x) \cdots (1 - s^{-l}x) } \notag\\
& = \sum_{k} c_k^{(k+l) } x^k  \label{generating function}
\end{align}
We prove by induction on $l$. For $l = 0$ this is obvious. Assuming case $l$ is correct, consider case $l+1$: 
\begin{align*}
	f^{(l+2)}(-x) 
	& = \frac{1}{1 - s^{-(l+1)}x}f^{(l+1)} (sx)\\
	&   \stackrel{\text{by induction hypothesis}}{=} (1 + s^{-(l+1) x }  + \cdots) \sum_k c_k^{(k+l)} s^k x^k \\
	& = \sum_N x^N \sum_{k=0}^{N} c_k^{(k+l)} s^{-(l+1)(N-k) + k} 
\end{align*}
Repeatedly use the relation 
$$
c^{(d+1)}_N = s^N c_N^{(d)} + s^{N-d-1} c_{N-1}^{(d)},  
$$
one can show
$$
c_N^{(N+l+1)} = \sum_{k=0}^{N} c_k^{(k+l)} s^{-(l+1)(N-k) + k}
$$
Thus \eqref{generating function} is also true for $l+1$. 


\end{proof}


Then consider case $P_{-\y}$:
\begin{align*}
	\Ad_{Q_\x} \Ad_{Q_\y} \cdot P_{-\y} 
	&= \Ad_{Q_\x} \cdot P_{-\y}\\
	&= \sum_{k\geq 0} (-1)^k P_{k \x -y}
\end{align*}
while
\begin{align*}
	\Ad_{Q_\y} \Ad_{Q_{\x + \y }} \Ad_{Q_\x} P_{-\y} 
	&= \Ad_{Q_\y} \Ad_{Q_{\x + \y }} \sum_{k\geq 0} (-1)^k P_{k\x - \y} \\
	&= \Ad_{Q_\y} \sum_{k, l\geq 0} (-1)^k c_l^{(-k-1) }  P_{(k+l) \x + (l-1) \y }\\
	&= \sum_{k, l, t \geq 0} (-1)^k c_l^{(-1-k)} c_t^{(-(k+l))} P_{(k+l)\x + (l+t)\y -\y}
\end{align*}

Compare the $P_{M\x + N\y -\y} $ term, we need show:
\begin{equation}
	\sum_{0\geq l \geq M } (-1)^{M-l} c_l^{(-M+l-1)} \cdot c_{N-l}^{(-M)}  = 0, \ \ \ \text{for}\  M\geq 0, N> 0.
\end{equation}
Using \eqref{x}, $c_l^{(-M+l -1)} = (-1)^{l} c_l^M$. Thus the above is equivalent to 
$$
 \sum_{0\leq l \leq M} c_l^M c_{N-l} ^{(-M)} = 0, \ \ N>0.
$$
This follows from the fact $f^{(M)} \cdot f^{(-M)} = 1$. 
\\



\todo[inline, color=blue!30]{still need to figure out the center of $\widehat{Sk(T^2)}$...}


\subsection{The face relation and skein-valued cluster transformation}

We consider a weave graph $\Gamma$ on $S^2$. Denote by $\Lambda_\Gamma$ the corresponding Legendrian, $L$ some Lagrangian filling. \cite{SS23} showed the wave function $\Phi_L$, taking value in $\widehat{Sk(L)}$, is annihilated by the ``face relation'':

\begin{align}\label{face relation}
	A_{\Gamma, F, v} \coloneqq   \pm \bigcirc \pm P_{e_1} \pm P_{e_1 + e_2} \pm \cdots \pm P_{e_1 + \cdots +e_{n-1}} 
\end{align} \todo[inline]{We already take $a = 1$ in the skein algebra. The signs here are given by the $\sigma$ in their paper, determined by the spin structre. Need to figure out those signs...}

\todo[inline]{As is pointed in Remark 7.2 of \cite{SS23}, we do not know how \eqref{face relation} depends on the choice of starting vertex $v$...}

were $F$ is a face of $\Lambda_\Gamma$, surrounded by edges $e_1, e_2, \ldots, e_n$, and $v$ is the vertex this face relation starts. 
 $P_{e}$ is the class in $Sk(\Lambda)$ represented by $ e $. 
 

 
 Let $e$ and $e'$ be two oriented simple closed curves, transversely intersecting at a single point. Then $e + e'$ can be defined as the ``connected sum'' of the two curves. 


As in the torus case, we can define ``Baxtor operators'' $Q_e \coloneqq  \E (\frac{P_e}{q^{1/2} - q^{-1/2}})$, and show
$$
\Ad_{Q_e} \cdot P_{e'}=
\left\{
\begin{array}{lr}
  (1 + \hat{e} ) P_{e'} ,  &\text{if }  (e, e') = 1, \\
  (1+\hat{e}^{-1})^{-1} P_{e'} = \sum_{k\geq 0} (-1)^k P_{e' - ke},  &\text{if } (e, e') = -1 .
  
  
\end{array}
\right.
$$
Here $\hat{e}$ is the operator sending $P_x$ to $P_{e+x}$. 

We want to show a similar result to Thm 4.3 of \cite{SSZ}. We use the same setting in figure (4.2.3) of \cite{SSZ}. Since $X_{e_1'} \stackrel{\mu_0}{ \longrightarrow} X_{e_1}(1+qX_{e_0}) = (1 + \hat{e}_0) X_{e_1} $ and $X_{e_2}'\stackrel{\mu_0}{\longrightarrow} X_{e_2}(1+qX_{-e_0} )^{-1} = (1 + {\hat{e}^{-1}_0} )^{-1} X_{e_2}   $. We would guess that 
\begin{align*}
	P_{e_0'}  &\stackrel{\mu_0}{\longrightarrow} P_{-e_0}\\
	P_{e_i'} &\stackrel{\mu_0}{\longrightarrow} {Q_{e_0}} \cdot P_{e_i}  
\end{align*}
Then we can try to do a similar computation as in the proof of \cite{SSZ} Thm 4.3:
\begin{align*}
	\mu_0(P_{e_2'} + P_{e_2' + e_0'}) &= \mu_0(P_{e_2'} + \frac{1}{\{-1\}}[P_{e'_2}, P_{e_0'}] ) \\
	& = \sum_{k \geq 0} (-1)^k P_{e_2 - ke_0} + \frac{1}{\{-1\}} [\sum_{k\geq 0}(-1)^k P_{e_2 - ke_0} , P_{-e_0} ]\\
	& = \sum_{k \geq 0} (-1)^k P_{e_2 - ke_0} + \sum_{k \geq 0} (-1)^k P_{e_2 - (k+1)e_0}\\
	& = P_{e_2} 
\end{align*}
\begin{align*}
	\mu_0(P_{e_2' + e_0' +e _1'}) 
	& = \frac{1}{\{-1\}}\mu_0 ([P_{e_2' + e_0'} , P_{e_1'} ] )\\
	& = \frac{1}{\{-1\}}[\sum_{k \geq 0} (-1)^k P_{e_2 - (k+1)e_0}, P_{e_1} + P_{e_1 + e_0} ]\\
	& = \sum_{k\geq 0} (-1)^k \frac{\{ - (k+2)\}}{\{-1\}} P_{e_2+e_1 -(k+1) e_0} + \sum_{k\geq 0} (-1)^k \frac{\{-(k+1)\}}{\{-1\}} P_{e_2 + e_1 - ke_0} \\
	& = P_{e_2 + e_1}
\end{align*}

\todo[inline]{This sounds stupid, but I feel we need to first understand what we are calculating here... I would guess $\mu_0$ should be viewed as some generalized "cluster transformation" between $\widehat{Sk(\Lambda_{\Gamma'}) } $ and $\widehat{Sk(\Lambda_\Gamma)}$? But maybe we want to know how (or whether) it is well defined... Then perhaps the above calculation (or something similar) would show that those the face relations $A$ are preserved by $\mu$}




